Reliable Cellular Automata with Self-Organization

In a probabilistic cellular automaton in which all local transitions have positive probability, the problem of keeping a bit of information indefinitely is nontrivial, even in an infinite automaton. Still, there is a solution in 2 dimensions, and this solution can be used to construct a simple 3-dimensional discrete-time universal fault-tolerant cellular automaton. This technique does not help much to solve the following problems: remembering a bit of information in 1 dimension; computing in dimensions lower than 3; computing in any dimension with non-synchronized transitions. Our more complex technique organizes the cells in blocks that perform a reliable simulation of a second (generalized) cellular automaton. The cells of the latter automaton are also organized in blocks, simulating even more reliably a third automaton, etc. Since all this (a possibly infinite hierarchy) is organized in ``software'', it must be under repair all the time from damage caused by errors. A large part of the problem is essentially self-stabilization recovering from a mess of arbitrary size and content. The present paper constructs an asynchronous one-dimensional fault-tolerant cellular automaton, with the further feature of ``self-organization''. The latter means that the initial configuration does not have to encode an infinite hierarchy -- this will be built up over time. This is a corrected and strengthened version of the journal paper of 2001.

==> tex-figures/fig-defs.tex <==
\setlength{\unitlength}{1pt}
\def\killtext#1{}

\newcommand{\latConf}{
 \begin{picture}(0,0)
   \newcommand{\SP}{\hspace{30pt}}
   \def\thn ##1{\makebox[0pt]{##1}}

   \put(0,60){\line(1,0){200}}
   \put(0,10){\line(1,0){200}}
 
   \multiput(43,58)(30,0){5}{\line(0,1){4}}

   \put(43, 45){\makebox{\thn{$0$}\SP\thn{$1.5$}\SP\thn{$3.0$}\SP
   \thn{$4.5$}\SP\thn{$6.0$}}}
   \put(43,70){\makebox{\thn{b}\SP\thn{u}\SP\thn{t}\SP\thn{o}\SP\thn{r}}}

   \put(260, 60){\makebox[0pt][l]{lattice configuration}}

   \multiput(13,8)(30,0){3}{\line(0,1){4}}
   \put(113,8){\line(0,1){4}}
   \put(143,8){\line(0,1){4}}

   \put(13,-5){\makebox{\thn{$-1.5$}\SP\thn{$0$}\SP
   \thn{$1.5$}\hspace{40pt}\thn{$3.5$}\SP\thn{$5.0$}}}

   \put(13, 20){\makebox{\thn{b}\SP\thn{u}\SP
   \thn{t}\hspace{40pt}\thn{o}\SP\thn{r}}}

   \put(260, 10){\makebox[0pt][l]{non-lattice configuration}}
 \end{picture}}

\killtext{
 \begin{figure}
   \begin{picture}(300, 80)
     \put(0,20){\latConf}
   \end{picture}
   \caption{Lattice configuration, non-lattice configuration}
 \end{figure}
}




